A Framework for Fast Polarity Labelling of Massive Data Streams

Many of the existing sentiment analysis techniques are based on supervised learning, and they demand the availability of valuable training datasets to train their models. When dataset freshness is critical, the annotating of high speed unlabelled data streams becomes critical but remains an open problem. In this paper, we propose PLStream, a novel Apache Flink-based framework for fast polarity labelling of massive data streams, like Twitter tweets or online product reviews. We address the associated implementation challenges and propose a list of techniques including both algorithmic improvements and system optimizations. A thorough empirical validation with two real-world workloads demonstrates that PLStream is able to generate high quality labels (almost 80% accuracy) in the presence of high-speed continuous unlabelled data streams (almost 16,000 tuples/sec) without any manual efforts.

==> 3_challenges.tex <==
\section{Motivation and Challenges}
\label{sec:challenges}
Driven by the widely deployed 5G and IoT technologies, we envision that online machine learning will soon become a mandatory task for every application, such as sentiment classification. In this regard, this work is a fundamental step towards the success of practical massive online machine learning.
In this section, we motivate our massive online sentiment classification with two concrete real-world use cases and summarize the corresponding design challenges.

\subsection{Example Use Cases}
Most existing sentiment classification approaches are based on offline batch-based learning mechanisms.
However, the demand for online sentiment classification is increasing fast.
% The motivations for online Sentiment Analysis are: 
First, 
the content and habits of people expressing opinions on social media are changing rapidly.
A model that is trained and updated with real-time data streams can intuitively respond to these changes better as we do not need to wait until all the data is collected before model training. This allows us to provide timely insights much earlier than relying on offline learning approaches.
% . Specifically, different from offline approaches, we do not wait until all the data is collected before model training. As a result, we can provide timely insights much earlier than before. 
Second, 
online sentiment classification could also allow us to reduce data footprint as we can potentially drop irrelevant data early and continuously. This is particularly important if we want to deploy sentiment analysis services close to the users (e.g., on their mobile phone).
In the following, we describe two selected use cases as examples. 
% We now describe two selected use cases as examples. 

\textbf{Feedback to Epidemic Outbreak.} 
Understanding the way ideas, innovations, behaviors, and diseases propagate over social networks is of considerable importance to the enabling of early warning as to the emergence of violence or outbreak of an epidemic. 
Previous work has attempted sentiment analysis~\cite{dubey2020twitter} on Twitter datasets to analyze how the citizens of different countries are dealing with the outbreak of COVID-19. 
In particular, it was discovered that while the majority of people throughout the world are taking a positive and hopeful approach, there are instances of fear, sadness, and disgust exhibited worldwide. Some countries have shown signs of distrust and anger on a larger scale as compared to others. 
Our envisioned massive online sentiment classification can be used in a much finer-grained manner compared to existing offline approaches. 
For example, it can be applied to real-time analysis of local and regional information (e.g., residences on a particular street) that can help the authorities take proper actions accordingly immediately.

\textbf{Financial Crime Detection.} 
Security breaches have been arising issues that cast a large amount of financial losses and social problems to society and people. In particular, unusual patterns/events of security breaches can be detected in the early stage, which could prevent further destruction by raising public awareness. 
Prior studies have shown that social media could be used a surveillance tool to track messages related to security breaches~\cite{hao2016social}. 
A framework has been proposed where the 113,340 were extracted, related to consumer security breach. 
A time-series analysis is performed that presents significant trends for various topics, and the sentiment analysis results show a considerable difference among the various topics. It confirms the usefulness in shaping public perception and guide companies on how to respond to consumer security breaches. 
The massive online sentiment classification can be applied in such a case with further improved performance, e.g., lower detection latency, and can be used to analysis much large size of datasets compared to existing works.
% This work is useful in shaping public perception and guide companies on how to respond to consumer security breaches. 
% The limitation with this is that the dataset collected from Twitter is for a short duration and covers only five topics in particular. The sentiment analysis algorithm and the techniques used are not discussed, and no comparison with other works is presented.

% \begin{myenumerate}
%     \item \textbf{Cyber Event Detection.} 
%     Cyber threats are hard to identify and predict because the hackers that conduct these attacks often obfuscate their activity and intentions. However, they may still use publicly accessible forums discuss vulnerabilities and share tradecraft about how to exploit them. The behavior of the hacker community, as expressed in such venues, may provide insights into group’s malicious intent~\cite{deb2018predicting}. To this end, the proposed project can be applied to predict malicious cyber events by exploiting malicious actor’s behavior via sentiment analysis of posts on hacker forums.

%     \item \textbf{Feedback to Epidemic Outbreak.} 

%     \item \textbf{Early Protest Detection.} National security analysts and officials have expressed interest in understanding public sentiment~\cite{colbaugh2011agile}. For example, beginning on 25 January 2011, a popular uprising swept across Egypt in the form of massive demonstrations and rallies, labor strikes in various sectors, and violent clashes between protestors and security forces, ultimately leading to the resignation of Egyptian President Hosni Mubarak on 11 February. It is ideal if we can discover the public sentiment regarding the Egyptian revolution generally and Mubarak specifically, especially 1.) in the weeks before the protests and 2.) for different regions of the globe. http://www.saujs.sakarya.edu.tr/en/download/article-file/1028640
    
%     \item \textbf{Financial Crime Detection.} Security breaches have been arising issues that cast a large amount of financial losses and social problems to society and people. In particular, unusual patterns/events of security breaches can be detected in the early stage, which could prevent further destruction by raising public awareness. Prior studies have shown that social media could be used a surveillance tool to track messages related to security breaches~\cite{hao2016social}. A framework has been proposed where the 113,340 were extracted, related to consumer security breach. A time-series analysis is performed that presents significant trends for various topics, and the sentiment analysis results show a considerable difference among the various topics. This work is useful in shaping public perception and guide companies on how to respond to consumer security breaches. The limitation with this is that the dataset collected from Twitter is for a short duration and covers only five topics in particular. The sentiment analysis algorithm and the techniques used are not discussed, and no comparison with other works is presented.
% \end{myenumerate}

\subsection{Design Challenges}
Motivated by the aforementioned applications, our ultimate design goal is to achieve high accuracy unsupervised sentiment classification of massive volume of social data streams.
We identify that there are three major challenges of achieving the goal.

\begin{myitemize}
    \item \textbf{Challenge 1: One Pass Incremental Learning.}
    In contrast to existing offline algorithms that learn once from a large collection of datasets, our algorithm must be able to continuously learning from new data. 
    First, pre-trained models in a majority of previous work of sentiment analysis would be limited to the knowledge from the training datasets and is incapable to adapt to new words.
    Second, considering the huge amount of data storage and transmission overhead, we simply cannot collect all the data sources before analysing due to the limitation in hardware resources (e.g., memory). As a result, the algorithm is required to only visit the input data once and nearly only once.
    % For example, the words express feeling might be different as time goes by~\cite{10.1145/2064448.2064475}, i.e. semantic change. 
    %  In contrast to existing offline algorithm, one of the challenges is that our algorithm must be able to continuously learning with new data. 
    % In a majority of previous work of sentiment analysis, the model is once trained and never updated/retrained anymore, i.e. the model is limited to the knowledge from the training datasets we feed to it and is incapable to adapt to the fast changing world. For example, the words people express their feeling might be different as time goes by. 
    %  Besides that, it is generally assumed that the training data has already been collected while we have to train the model with real time data stream in online scenario. 
    % Furthermore, 
    Such one pass incremental sentiment analysis still remains an open and challenging problem up to date.
    
    \item \textbf{Challenge 2: Lack of Labels in Training Datasets.} 
    To achieve high prediction accuracy for sentiment classification is a notorious challenge~\cite{6996998,VASHISHTHA2019112834,rahnama2014distributed,smailovic2014stream}, and many novel algorithms been studied in the recent years~\cite{56622554082144859b6c5cf5ff238ad8}. Despite the success of prior works to achieve high accuracy in sentiment classification, we observe that they are mostly based on supervised learning paradigm. The cost to acquire ground true label could be expensive (if not impossible) in the real-world scenario. Moreover, it is difficult to keep the training datasets relevant as how people expressing opinions on social media changes frequently over time, e.g., there are many ``internet slang" appear every year. Hence, fully unsupervised algorithms are highly desired but are less studied for sentiment analysis. A few prior studies leverage on simple clustering mechanism~\cite{Zimmermann:NeuroComp14} to achieve unsupervised or semi-supervised sentiment analysis but are shown to have a low accuracy in general cases as we will demonstrate in our experiments.

    \item \textbf{Challenge 3: High Velocity of Input Streams.} 
    We need to handle large volume of data streams during sentiment classification. For example, there are around 10,000 tweets per second according to twitter usage statistics~\cite{twitter}. Prior solutions are mostly emphasized at only algorithmic accuracy and are not able to utilize the more and more abundant parallel hardware resources. Although general-purpose data stream processing systems such as Apache Flink~\cite{carbone2015apache} can provide fast stream processing capability, it still remains an open question of how to leverage them to achieve high performance sentiment analysis, e.g., it is still a challenging task to efficiently manage and update the learned embedding model over a highly parallelized run time.
\end{myitemize}

==> 9_background.tex <==
\section{Background}
\label{sec:background}
% We now provide key definitions and terminology, which will be used throughout the paper. 
% \cc{We summarize the notations used throughout this paper in Table~\ref{}.}
In this section, we introduce preliminary knowledge on online sentiment learning, word embedding, and data stream processing systems (DSPSs). 
We summarize the notations used throughout this paper in Table~\ref{tab:notations}.
% first define online sentiment classification.
% Then, we introduce preliminary knowledge of data stream processing systems (DSPSs).
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Notations used in this paper. Parameter value ranges used in our experiments are also shown.}
\label{tab:notations}
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{|p{1.5cm}|p{2.8cm}|p{6.2cm}|}
\hline
Name         & Notation & Description                                                                     \\ \hline
Tuple        & $T=\{t, v_1, v_2, ..., v_n\}$        & A timestamped ($t$) finite number $n$ of words ($v_i$) with a polarity to be identified \\ \hline
Input stream & $S=\{T_1, ..., T_N\}$     & A list of tuples chronologically arriving at the system to be analyzed \\ \hline
% Batch        & $B=<T_1, ..., T_b>$     & A list of tuples to be processed where the list size ($b$) is tunable                                                                               \\ \hline
Weight Matrix & $M_{m,d}$, where each element in $M$ is denoted as $m_{i,j}$  & The vector representation of a list of words, where $m$=number of words, and $d$=number of features                                                                \\ \hline
Vector lookup table        & $V: word \rightarrow m_{i}$    & A lookup table of trained word (key) with corresponding vector representation in $M$ (value)                                                                         \\ \hline
Window        & $w=1\sim10$     & A tunable training window size used by Word2Vec to capture contextual information                                                                              \\ \hline
Vector Dimension        & $d=10\sim500$     & A tunable feature size used by Word2vec training                                                                    \\ \hline
Batch size        & $b=200\sim5000$     & A tunable size of batched tuples being collected before training                                                                    \\ \hline
Minimum Word Count        & $MWC=1\sim20$     & A tunable size used by Word2vec to determine how much time a word at least should appear before being fed to training.                                                                     \\ \hline
Trend Detection Window        & $TDW=200\sim2000$     & A tunable window size for polarity trend detection                                                                               \\ \hline
Model Merging Periodic       & $p=20\sim90 (seconds)$     & Model merging frequency                                                                              \\ \hline
LRU Cache Size       & $c=30000\sim50000$     & The cache size threshold of LRU pruning                                                                              \\ \hline
% Weighted coefficient        & $WC=0\sim1$, the adjustment step size $\delta$ is also tunable    & Adjustable weighted coefficient in cosine similarity calculation according to polarity trend detection                                                                   \\ \hline
\end{tabular}%
}
\end{table}

\subcompact
\subsection{Online Sentiment Learning}
% \subsection{Sentiment Classification}
% Among various opinion mining tasks, one of them is sentiment classification, i.e. whether the semantic orientation of a text is positive, negative or neutral.
Sentiment classification is an application of natural language processing (NLP) that analyzes subjective texts with emotions to determine the views, preferences, and tendencies of a text.
% In particular, it determines whether the semantic orientation of a text is positive, negative or neutral. 
Most prior works~\cite{2016Machine,go2009twitter,gautam2014sentiment,haque2018sentiment,ortigosa2014sentiment} belong to \emph{offline sentiment learning}, which typically requires a \emph{training} phase that trains a classifier with labelled training texts followed by an \emph{inference} phase that identifies the polarity of a testing text based on the trained classifier.
% leverage machine learning methods~\cite{2016Machine}. 
% They typically require a \emph{training} phase which trains a classifier with labelled training texts followed by a \emph{inferring} phase which identify the polarity of a testing text based on the trained classifier.
% For example, through sentiment classification of user reviews on shopping websites, user satisfaction with products can be quickly analyzed, thereby helping individuals or companies to adjust product strategies. 
Their primary concern is to obtain a high accuracy classifier from a large set of collected and labelled datasets, assuming infinite time and resource budgets.
In contrast, we focus on \emph{online sentiment learning} that learns and identifies the polarity of ongoing data streams at one phase. 
Specifically, we define a \emph{tuple} (denoted as $T$) as a timestamp $t$ associated with a
finite number of vocabularies (i.e., $v_1\sim v_n$). 
% and a timestamp (i.e., $t$).
The \emph{input stream} is a list of tuples chronologically arriving at the system, denoted as $S=\{T_1, ..., T_N\}$, where $N$ goes to infinity.  
Then, we can define online sentiment learning as follows.
\begin{definition}
Given an input stream $S$,
\textbf{online sentiment learning} is the process used to learn and identify the polarity of $T_i \in S$ as soon as $T_i$ arrives without relying on any offline training phase with labelled datasets. 
\end{definition}

% Differ significantly from the offline sentiment learning, 
It is noteworthy that the classifier trained by online sentiment learning is continuously updated, as both the vocabulary and the polarity model evolve. 
% making pre-trained classifier quickly become outdated.
In other words, every input tuple 
% for online supervised sentiment classification 
functions as both the \emph{training} and \emph{testing} dataset.
This differs significantly from offline sentiment learning, where the pre-trained classifier can quickly become outdated. Due to significant differences in problem assumptions, we do not further compare our solution with existing offline approaches. 
Instead, we extensively evaluate several alternative online approaches, including those that rely on stream clustering mechanisms~\cite{Zimmermann:NeuroComp14}.
% from on-going unlabelled data streams 
% To the best of our knowledge, how to preserve the high accuracy of sentiment classification while achieving high throughput and low latency in processing large-scale unlabeled data streams such as social media opinions, so far has been an unsolved problem. 
% In this work, we present the first attempt towards online unsupervised sentiment classification, which will be discussed in detail in Section~\ref{subsec:preprocess} and Section~\ref{subsec:learning}.

% As a result, most existing offline sentiment classification methods are incapable to be applied for analyzing
% streams consist of unbounded, non-stationary data objects that continuously arrive at rapid rates
% In application scenarios that require low latency processing, such as stock trading, online sentiment classification can provide transaction decision support. 
% However, most sentiment analysis methods are batch-based and not applicable to analyze the public reaction on articles in real-time, as streams consist of unbounded, non-stationary data objects that continuously arrive at rapid rates. Their intrinsic nature requires algorithms capable of processing data and extracting knowledge under the challenges of limited time, memory, and requires only single pass (i.e., allow nearly no revisit of the input data).


% To analyse the unstructured natural language text, we need to first convert them into numeric values. The training step is to learn the vector representation of each word of the input streams. Context-free models such as Word2vec (W2V) or GloVe generate a single word embedding representation for each word in the vocabulary, where the recently proposed BERT takes into account the context for each occurrence of a given word.  The former can train much faster than the latter while BERT may be able to generate vector representations with more valuable contextual information. However, neither has been examined in the proposed novel context: training directly on continuously in-coming stream data points. To this end, we propose to combine the idea of contextual-aware embedding (i.e., BERT) and static embedding (i.e., W2V). Specifically, we use W2V for text vectorization as it is suitable for online learning since it can update the vector representation of each vocabulary incrementally with only local data sets, i.e., the current input tuple being processed. Once the neural network is trained, the weight matrix M_(m,d) is taken as the learned vector representation, where m=number of distinct words seen so far, and d=number of features in the hidden layer. We denote each element in M as m_(i,j),where i indicates which word, and j indicates which feature. To allow W2V to capture more contextual information, we aggregate representation of each word from multiple input tuples through sampling on the input streams as contexts. A pooling (i.e., min, max, mean) strategy is then applied to yield a single representation that aggregates across contexts. 
\subcompact
\subsection{Word Embedding}
\label{subsec:embedding}
To analyze unstructured natural language texts, a common step is to first convert vocabulary into a vector of numeric values, usually called \emph{word embedding}.
Two classical word embedding algorithms are \emph{one-hot encoding} and \emph{bag of words}~\cite{birunda2021review}. However, one-hot encoding will lead to a dimension explosion when the vocabulary size becomes larger, while bag of words does not consider the context information in one sentence. 
% Natural language text is unstructured. In order to extract features from such data, one-hot encoding and bag of words are two common and popular text vectorization algorithms.
Representative recent approaches to word embedding include \emph{word2vec}~\cite{mikolov2013efficient}, \emph{Glove}~\cite{2014Glove}, \emph{BERT}~\cite{devlin2018bert} and their variants~\cite{10.5555/3044805.3045025}.
\emph{Glove}~\cite{2014Glove} combines local contextual information with overall statistics of the corpus, while \emph{BERT}~\cite{devlin2018bert} uses MLM (mask language model) for pre-training and uses deep bidirectional transformer~\cite{vaswani2017attention} components to build the entire model with bidirectional contextual information, i.e., each word has different vector representations in different context.
Despite their effectiveness, both the training of \emph{Glove} and \emph{BERT} are batch-based, requiring the presence of the entire input datasets and cannot be applied to learn from on-going input streams. 
In contrast, \emph{word2vec} is able to capture the vector representation of each vocabulary incrementally with local information. 
Specifically, a window ($w$) of a predefined length is moved along vocabularies (called \emph{corpus}) of each input tuple. In each step, the network is trained by predicting a word by referencing other words inside the same window. This allows word2vec to be trained incrementally upon the receipt of each input tuple, and thus satisfy the requirements of online sentiment learning. 
% our goal of achieving online sentiment learning.  
% We hence express the word embedding process in this work as follows.
% \begin{definition}
%     Given an input tuple $T$, \textbf{incremental word embedding} in our system is a process to train a neural network by taking each $v_i$ as the predicting target vocabulary, and the neighbours $v_{i-w/2}$, $v_{i-w/2+1}$, ..., $v_{i+w/2}$ as the training vocabularies. 
%     Once the neural network is trained, we will obtain a weight matrix (or called ``model'') $M_{m,d}, where\ m=\text{number of distinct words},\ \text{and}\ d=\text{number of features}$ in the hidden layer. Each row in $M$ is then a \textbf{vector representation} of a vocabulary. We denote each element in $M$ as $m_{i,j}$, where $i$ indicates which word, and $j$ indicates which feature.
% \end{definition}
Nevertheless, word2vec was not specifically designed for training over data streams. 
There are two major limitations of word2vec in applying to online sentiment learning. 
First, the original word2vec considers only contextual information within a sentence and overlooks the temporality among input tuples in the data streams, which carries important chronological information. 
Second, the size of the weight matrix $M$ (i.e., the word embedding results) trained by word2vec can continuously grow with the learning of new data and eventually cause the system to no longer be able to make progress.
We will discuss how we apply word2vec in our system and address those limitations in detail later in Section~\ref{subsec:learning}.

\subcompact
\subsection{Data Stream Processing Systems}
In the last decade, data stream processing systems (DSPSs) have received considerable attention. Many DSPSs have been proposed, such as Apache Flink~\cite{carbone2015apache}, Apache Storm~\cite{ApacheStorm}, and Spark Streaming~\cite{Sparkstream}.
% With the explosion of information, being able to process data streams efficiently in real time is perceived as a major challenge. 
% In addition to being compatible with various data sources and having multiple options for storing processing results, the core of a DSPS should be the reliable data stream processing engine. 
% At present, Apache Flink~\cite{carbone2015apache}, Apache Storm~\cite{ApacheStorm}, Spark Streaming~\cite{Sparkstream} are three well-known DSPSs.
In this study, we leverage Apache Flink for stream processing due to its capability of expressive, declarative, and efficient data analysis on data streams~\cite{carbone2015apache}, with high-level programming language API support such as the Python API~\cite{pyflink}. 
% It can be deployed in various cluster environments to quickly calculate data in various scales.
% Different from Storm and Spark streaming, Flink is not only a high-throughput, low-latency stream processing engine, but also supports window operations with event time, stateful calculation, window functions and advanced operators. 
Nevertheless, our proposed solution is general and can be applied to other DSPSs with similar characteristics. 
% spending marginal programming efforts.
% In addition, Flink has added support for Python since version 1.9.0~\cite{pyflink}, which means that Python's popularity in Data Analysis/AI researching can be combined with Flink.
% This will provide more possibilities for Flink in future machine learning research.
% However, modern DSPSs including Apache Flink are not specifically designed for online machine learning such as 
% In this work, we carefully revise and optimize sentiment classification algorithms towards online unsupervised learning, which will be discussed in detail in Section~\ref{subsec:preprocess} and Section~\ref{subsec:learning}.
% are remaining as an open and challenging question, which will be answered in this work.
% In this work, we adopt Flink for its well-known high throughput and low latency performance in handling continuous data streams. 
% Therefore, deploying machine learning algorithms on SPEs such as Apache Flink is now still a popular and open research problem.
% \subsection{Key Value Store}
However, a major limitation of modern DSPSs is the lack of support for \emph{shared mutable state}~\cite{tstream}, i.e., a shared memory that multiple application threads can access and update concurrently.
% e.g., shared application states where multiple threads spawned from the same application can reference and update at the same time. 
Shared state is crucial for the task of online sentiment learning as parallel training requires multiple threads to access and update the trained model. 
This is not supported by Flink by default.
% sentiment classification training task as when the streaming tweets are processed in a parallel way, different tweet processing threads may need to access the same learned embedding model for updating or inference, which is not supported by Flink by default.
% The common wisdom is to rely on a key-value store 
Commonly, one will leverage a key value store (KVS) to maintain such shared mutable states for stream processing. 
Typical examples of such KVS systems include
% and there are many key-value store solutions available such as 
Redis~\cite{redis} and RocksDB~\cite{rocksdb}.
% In this work, we use Redis for storing the learned embedding model.
% so that different threads can access the shared learned model. 
As our experimental results will demonstrate, naively relying on a KVS to manage the access and update of a trained classifier leads to a huge run-time overhead. 
As a result, we adopt several state management optimization techniques in \system, which will be discussed in detail in Section~\ref{subsec:model_management}.
% Nevertheless, it is still an interesting topic to further explore the potential usage of more advanced solutions of shared mutable state management of stream processing such as transactional state management~\cite{tstream}, which could potentially improve both accuracy and performance of \system. Due to its significant complexity, we leave it as a future work.
 


==> Materials.tex <==
Unfortunately, this poses significant challenges that make existing solutions no longer adequate. Specifically, 
% \subsection{Design Challenges}
% Motivated by the aforementioned applications, our ultimate design goal is to achieve high accuracy unsupervised sentiment classification of massive volume of social data streams.
% We identify that there are three major challenges to achieve massive online sentiment classification.
% . of achieving the goal.
\begin{myitemize}
    \item \textbf{Challenge 1: One-pass Incremental Learning.}
    Most existing works~\cite{go2009twitter,gautam2014sentiment,haque2018sentiment,ortigosa2014sentiment} are geared towards analysis based on offline learning. Essentially, they assume unlimited time and resource budgets to extract information from collected datasets as much as possible.
    In contrast, we need to visit the input data once and nearly only once without storing the fast ongoing data streams. 
    % need to continuously learn from fast on-going data streams, and the algorithm is required to only visit the input data once and nearly only once.  
    % For example, the words express feeling might be different as time goes by~\cite{10.1145/2064448.2064475}, i.e. semantic change. 
    %  In contrast to existing offline algorithm, one of the challenges is that our algorithm must be able to continuously learning with new data. 
    % In a majority of previous work of sentiment analysis, the model is once trained and never updated/retrained anymore, i.e. the model is limited to the knowledge from the training datasets we feed to it and is incapable to adapt to the fast changing world. For example, the words people express their feeling might be different as time goes by. 
    %  Besides that, it is generally assumed that the training data has already been collected while we have to train the model with real time data stream in online scenario. 
    % Furthermore, 
    To the best of our knowledge, to achieve such one-pass incremental sentiment learning still remains an open and challenging problem. %as of today. 
    % These works assume a large amount of datasets are being collected beforehand. Offline learning introduced significant delay, especially if the analysis results have to be sent back to the data sources (e.g., mobiles) and they were not able to keep the trained model up to date.
    
    \item \textbf{Challenge 2: Lack of Labels in Training Datasets.} 
    % To achieve high polarity classification accuracy is a notorious challenge~\cite{6996998,VASHISHTHA2019112834,rahnama2014distributed,smailovic2014stream}, and many efforts have been devoted to improve the prediction accuracy in the recent years~\cite{56622554082144859b6c5cf5ff238ad8}. 
    Despite the success of prior works~\cite{VASHISHTHA2019112834,rahnama2014distributed,smailovic2014stream,56622554082144859b6c5cf5ff238ad8} at achieving high polarity classification accuracy, 
    % we observe that 
    they are mostly based on a supervised learning paradigm. 
    The cost of acquiring ground truth labels may be expensive (if not impossible) in real-world scenarios. In particular, 
    it is difficult to maintain relevant training data, since peoples' opinions change rapidly over time.
    % it is difficult to keep the training datasets relevant as how people express opinions changes frequently over time. 
    % Moreover, it is difficult to keep the training datasets relevant as how people expressing opinions changes frequently over time. 
    We therefore need to be able to perform sentiment learning without any training data.
    % Hence, fully unsupervised algorithms are highly desired but are less studied for sentiment analysis. 
    A few prior studies leveraged the clustering mechanism~\cite{Zimmermann:NeuroComp14} to achieve unsupervised or semi-supervised sentiment classification. However, we will demonstrate later in our experiments that they are unable to achieve satisfactory classification accuracy in general cases, and a new approach is thus required.
    
    % but are shown to achieve a low accuracy in general cases as we will demonstrate in our experiments.

    \item \textbf{Challenge 3: High Velocity of Input Streams.} 
    Prior solutions~\cite{56622554082144859b6c5cf5ff238ad8} mostly emphasize the improvement of theoretical performance bounds or the improvement of accuracy. 
    % They are not able to utilize the more and more abundant parallel hardware resources.     
    In contrast, we need to handle large volumes of data streams during sentiment learning. For example, there are around $10,000$ tweets per second, according to Twitter usage statistics~\cite{twitter}. 
    Although general-purpose data stream processing systems (DSPSs) such as Apache Flink~\cite{carbone2015apache} can provide fast stream processing capability, it remains an open question how to leverage them to achieve high performance sentiment learning. 
    % e.g., it is still a challenging task to efficiently manage and update the learned embedding model over a highly parallelized run time. 
    % We observe that prior work emphasize only improving theoretical algorithmic performance (e.g., prediction accuracy) and do not scale well in practice in terms of processing throughput and/or latency. 
    To the best of our knowledge, no work has attempted online sentiment learning in a modern parallel hardware environment.
\end{myitemize}

==> SIGMOD_BLOCK.tex <==
%%
%% \BibTeX command to typeset BibTeX logo in the docs
\AtBeginDocument{%
  \providecommand\BibTeX{{%
    \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

%% Rights management information.  This information is sent to you
%% when you complete the rights form.  These commands have SAMPLE
%% values in them; it is your responsibility as an author to replace
%% the commands and values with those provided to you when you
%% complete the rights form.
\setcopyright{acmcopyright}
\copyrightyear{2018}
\acmYear{2018}
\acmDOI{10.1145/1122445.1122456}

%% These commands are for a PROCEEDINGS abstract or paper.
\acmConference[Woodstock '18]{Woodstock '18: ACM Symposium on Neural
  Gaze Detection}{June 03--05, 2018}{Woodstock, NY}
\acmBooktitle{Woodstock '18: ACM Symposium on Neural Gaze Detection,
  June 03--05, 2018, Woodstock, NY}
\acmPrice{15.00}
\acmISBN{978-1-4503-XXXX-X/18/06}

==> vldb_block.tex <==
%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\pagestyle{\vldbpagestyle}
\begingroup\small\noindent\raggedright\textbf{PVLDB Reference Format:}\\
\vldbauthors. \vldbtitle. PVLDB, \vldbvolume(\vldbissue): \vldbpages, \vldbyear.\\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi}
\endgroup
\begingroup
\renewcommand\thefootnote{}\footnote{\noindent
This work is licensed under the Creative Commons BY-NC-ND 4.0 International License. Visit \url{https://creativecommons.org/licenses/by-nc-nd/4.0/} to view a copy of this license. For any use beyond those covered by this license, obtain permission by emailing \href{mailto:info@vldb.org}{info@vldb.org}. Copyright is held by the owner/author(s). Publication rights licensed to the VLDB Endowment. \\
\raggedright Proceedings of the VLDB Endowment, Vol. \vldbvolume, No. \vldbissue\ %
ISSN 2150-8097. \\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi} \\
}\addtocounter{footnote}{-1}\endgroup
%%% VLDB block end %%%

%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\ifdefempty{\vldbavailabilityurl}{}{
\vspace{.3cm}
\begingroup\small\noindent\raggedright\textbf{PVLDB Artifact Availability:}\\
The source code, data, and/or other artifacts have been made available at \url{\vldbavailabilityurl}.
\endgroup
}
%%% VLDB block end %%%
